Quantifying Semantic Query Similarity for Automated Linear SQL Grading: A Graph-based Approach

Quantifying the semantic similarity between database queries is a critical challenge with broad applications, ranging from query log analysis to automated educational assessment of SQL skills. Traditional methods often rely solely on syntactic comparisons or are limited to checking for semantic equivalence. This paper introduces a novel graph-based approach to measure the semantic dissimilarity between SQL queries. Queries are represented as nodes in an implicit graph, while the transitions between nodes are called edits, which are weighted by semantic dissimilarity. We employ shortest path algorithms to identify the lowest-cost edit sequence between two given queries, thereby defining a quantifiable measure of semantic distance. A prototype implementation of this technique has been evaluated through an empirical study, which strongly suggests that our method provides more accurate and comprehensible grading compared to existing techniques. Moreover, the results indicate that our approach comes close to the quality of manual grading, making it a robust tool for diverse database query comparison tasks.

==> src/basics.tex <==
\section{Basics}\label{sec:basics}

In this section, basic knowledge that will be relevant for the rest of this paper is provided.
Since the topic is "\title{}", the subjects here will be \ac{sql} and its queries (see \autoref{sec:sql}), the decidability of their comparison (see \autoref{sec:decidability}), and the shortest path problem (see \autoref{sec:shortest-path-problem}).


\subsection{SQL}\label{sec:sql}

\acs{sql} stands for \acl{sql}.
It is the standard language for relational \acp{dbms}. \cite[section 6]{Elmasri.2015}
A \ac{dbms} manages the creation of, maintenance of, and access to a database, which in turn is the underlying collection of related data. \cite[section 1.1]{Elmasri.2015}
Relational refers to the database consisting of tables, called relations.
Their columns are called attributes and the elements they contain are tuples with one value for each attribute.
This is visualized in \autoref{fig:relation-annotated}.

\begin{figure}[htb]
	\centering
	\includegraphics[width=0.7\linewidth]{fig/Relation-annotated}
	\caption{The relation \texttt{students} with its tuples and attributes.}
    \Description{A table with sample entries illustrating that an attribute is the name of a column, a tuple is a line, and the relation is the table in its entirety.}
\label{fig:relation-annotated}
\end{figure}

\ac{sql} contains statements for defining, modifying and querying data. \cite[section 6]{Elmasri.2015}
Since the latter one, namely the SELECT-query, is the most common and easy to understand, this paper will focus on it (without loss of generality, see \autoref{sec:generalizability}).
The query is made up of multiple clauses, the most important of which are listed in \autoref{lst:basic-query-clauses}.

\begin{lstlisting}[language=SQL, caption=Basic query clauses., label=lst:basic-query-clauses]
    [ WITH <with-element list> ]
    SELECT [DISTINCT] <select-element list>
    FROM <from-element list>
    [ WHERE <expression> ]
    [ GROUP BY <expression list>
    [ HAVING <expression> ] ]
    [ ORDER BY <order-by-element list> ]
\end{lstlisting}

The SELECT- and FROM-clause are mandatory, the others optional.
The query returns a multi-set of tuples.
Its SELECT-clause determines the number and content of their attributes.
If \texttt{DISTINCT} is specified, duplicate entries are eliminated, making the result a simple set, otherwise not.
A SELECT-element mainly consists of an expression, but additionally can be renamed with an alias, like so: \texttt{<expression> [AS] <alias>}.
In the FROM-clause, those tables / relations are listed, which contain tuples used by the query.
Therefore, a FROM-element is a table-reference, also with an optional alias.
Unlike before, this alias does not change the result of the query, but only the way the table is referred to inside the query.
Such an alias becomes necessary when the same table is used multiple times.
Also, FROM-elements may be joined with one another using an INNER, LEFT OUTER, RIGHT OUTER, or FULL OUTER JOIN.
In this case, a JOIN-condition must be specified, like so: \texttt{<from-element> [INNER | (LEFT | RIGHT) [OUTER] | FULL OUTER] JOIN <from-element> ON <expression>}.
The WHERE-clause decides whether a tuple is kept or discarded by interpreting its expression as a boolean value.
If there is a GROUP-BY-clause, tuples are put into groups depending on whether all of the listed expressions match for them.
The HAVING-clause works similar to the WHERE-clause, but on said groups instead of individual tuples.
And via the ORDER-BY-clause, the entries of the query result can be sorted.
An ORDER-BY-element consists of an expression and an order, either \texttt{ASC} for ascending or \texttt{DESC} for descending.
The WITH-clause is a list of subqueries with alias names, which can be used in the rest of the query by addressing this alias.

An expression can be a simple column-reference, asterisk or literal constant.
It can also be more complex and recursively contain other expressions, like an aggregation function, an arithmetic expression, or a logical comparison.
The asterisk \texttt{*} references all columns of all tables in the FROM-clause, or, if prefixed with the table name or alias of a certain FROM-element, all columns of this specific table.
A column-reference can be prefixed the same way to clarify which table it belongs to.
This becomes necessary when there are two or more columns with the same name among the referenced tables.

Instead of the textual description above, \ac{sql} queries can also be represented as an \acf{ast}.
Every component becomes a node, with its sub-components being its child nodes.
Irrelevant syntactic information, for example punctuation or parentheses, can be abstracted or omitted, hence the name \ac{ast}.
In this hierarchical form, the structure and content is easier to analyze and edit than it would be as text.
This is why it is the preferred representation in most software processing \ac{sql}, and why it will be used here as well.
Take for example the \ac{sql} query in \autoref{lst:relation-annotated-query}, based on the table \texttt{students} from \autoref{fig:relation-annotated}.
An \ac{ast} representation of it is shown in \autoref{fig:simple-ast}.

\begin{lstlisting}[language=SQL, caption=A query on the relation \texttt{students}., label=lst:relation-annotated-query]
    SELECT s.id AS ID
    FROM students AS s
    WHERE s.age > 21
\end{lstlisting}

\begin{figure}[htb]
	\centering
	\includegraphics[width=0.67\linewidth]{fig/Simple-AST.png}
	\caption{\acs{ast} of the query on the relation \texttt{students}.}
    \Description{A graph depicting the abstract syntax tree of the above query.}
\label{fig:simple-ast}
\end{figure}


\subsection{Decidability}\label{sec:decidability}

Query equivalence, and therefore also the more general query containment, has long been found to be generally undecidable. \cite[section 6.3]{Chu.2017b, Abiteboul.1995}

A problem is decidable \ac{iff} there is an algorithm, that decides it in finite time. \cite[section 2.2]{Abiteboul.1995}
This means, the algorithm terminates and returns whether the problem is true or false for a given parameter.
Opposed to that, \ac{iff} a problem is undecidable, any algorithm that decides the problem cannot be guaranteed to terminate.

This means in the case of query equivalence, there is no algorithm, that, given two queries as parameter, always terminates in finite time and returns whether they are equivalent or not.
There certainly are simple cases where it can be decided in finite time.
For example, the queries in \autoref{lst:simple-query-1} and \autoref{lst:simple-query-2} are instantly recognizable as equivalent to each other, while none of them are equivalent to \autoref{lst:simple-query-3}.
But with more complex queries, this quickly becomes harder, and in general, it cannot be decided in finite time. \cite[section 6.3]{Chu.2017b, Abiteboul.1995}

\begin{lstlisting}[language=SQL, caption=Simple query., label=lst:simple-query-1]
    SELECT *
    FROM students
    WHERE age > 21
\end{lstlisting}

\begin{lstlisting}[language=SQL, caption=Simple query equivalent to the previous one., label=lst:simple-query-2]
    SELECT *
    FROM students
    WHERE 21 < age
\end{lstlisting}

\begin{lstlisting}[language=SQL, caption=Simple query not equivalent to any of the two previous ones., label=lst:simple-query-3]
    SELECT *
    FROM students
    WHERE age < 21
\end{lstlisting}


\subsection{Shortest Path Problem}\label{sec:shortest-path-problem}

The shortest path problem is a problem of graph theory.
For this purpose, a graph is a set of nodes (also called vertices), some of which are connected pairwise via edges.
These edges can have weights / costs assigned to them.
It is uniform across all edges of a graph whether they are directed, discerning from which and to which node they lead, or not, being traversable in both directions.
A graph can be given in explicit form as a pair, consisting of the set of all nodes and the set of all edges.
Or it can be in implicit form, where these sets are not given outright from the beginning. Instead, there is a neighbor function, that, for a given node, calculates its neighbors and the costs of the respective edges to them.
\autoref{fig:simple-graph} shows an example for a directed graph with nodes and weighted edges.

\begin{figure}[htb]
	\centering
	\includegraphics[width=0.2\linewidth]{fig/Simple-graph.png}
	\caption{Simple graph consisting of five nodes and nine weighted edges.}
    \Description{A graph consisting of nodes A-E connected via weighted edges.}
\label{fig:simple-graph}
\end{figure}

The shortest path problem is to find the path from a start to a destination node, for which the sum of costs of its edges is the lowest.
For example, in the graph in \autoref{fig:simple-graph}, the shortest path from node $A$ to node $E$ is $A \to D \to C \to E$.
Dijkstra's algorithm is a famous algorithm for solving the shortest path problem.
However, in its commonly taught form, it cannot be applied to implicit graphs because it would need to know all nodes of the graph right from the beginning. \cite{Felner.2011}
Instead, uniform cost search can be used, which is shown in \hyperref[alg:ucs]{Algorithm \ref*{alg:ucs}}.

\begin{algorithm}
\caption{Uniform Cost Search}\label{alg:ucs}
\begin{algorithmic}[1]
\Require Start Node \texttt{s}
\State \texttt{distance[s] $\gets$ 0}
\State \texttt{UNVISITED.insert(s,\ 0)}
\While{\texttt{UNVISITED $\neq$ $\emptyset$}}
    \State \texttt{u $\gets$ UNVISITED.extract\_min()}
    \State \texttt{VISITED.insert(u)}
    \For{(Node, Cost) \texttt{(n,\ c) $\in$ Neighbors(u)}}
        \If{\texttt{n $\notin$ VISITED}}
            \If{\texttt{n $\notin$ UNVISITED}}
                \State \texttt{distance[n] $\gets$ distance[u] + c}
                \State \texttt{UNVISITED.insert(n,\ distance[n])}
            \Else
                \State \texttt{distance[n] $\gets$ min(distance[n],\ distance[u] + c)}
                \State \texttt{UNVISITED.update(n,\ distance[n])}
            \EndIf
        \EndIf
    \EndFor
\EndWhile
\end{algorithmic}
\end{algorithm}

It uses a priority queue called \texttt{UNVISITED}, which is initialized with the start node \texttt{s} at its distance of \texttt{0}.
While this queue is not empty, the node \texttt{u} with minimal distance is extracted.
Because it has the minimal distance, there can be no other path to it with a smaller one (assuming non-negative edge costs).
So it is added to the set of visited nodes, called \texttt{VISITED}, whose distances will not change anymore.
Then, its neighboring nodes, along with the cost of the respective edge, are determined via the neighbor function of the implicit graph.
For each neighbor, it is checked whether it has already been visited before, in which case it is skipped because the shortest path to it was already found.
Otherwise, it is either added to the priority queue with a tentative distance, in case it was undiscovered before.
Or, in case it was already discovered, its tentative distance is updated to a potentially smaller value by using \texttt{u} as an intermediate step along the path.

Every node, apart from the start node, is at first undiscovered.
It is discovered but still unvisited, as soon as one of its neighbors becomes visited, at which point it receives a tentative distance.
If more of its neighbors are visited before itself, its tentative distance may get updated to a smaller value.
When it is extracted from the priority queue and becomes visited, its tentative distance is the smallest one of all unvisited nodes, so there can be no shorter path to it using another unvisited node.
Its tentative distance becomes its final distance.

\autoref{fig:simple-graph-ucs} shows the steps of applying uniform cost search to the graph from \autoref{fig:simple-graph}, starting at node $A$.
The queue of discovered, but unvisited nodes with their tentative distances and the respective paths in the graph are colored blue.
The set of visited nodes with their final distances and the respective paths in the graph are colored purple.
Notice how the tentative distance of node $E$, as well as the path to it, change multiple times as shorter alternatives are discovered.

\begin{figure}[htb]
	\centering
	\includegraphics[width=\linewidth]{fig/Simple-graph-UCS.png}
	\caption{The steps of applying uniform cost search with start node $A$ to the simple graph.}
    \Description{[A], [A, B], [A, B, D], [A, B, D, C], [A, B, D, C, E]}
\label{fig:simple-graph-ucs}
\end{figure}

In the form described above, the algorithm builds a tree of shortest paths from the start node as root to every other node in the graph.
But often only the shortest path to one specific destination node is of interest.
In this case, the algorithm can be stopped as soon as this destination becomes visited, because its distance and path will not change anymore.
This is again assuming all edge costs are non-negative.
For example, if node $C$ from above was the destination, the algorithm could have stopped after step five.


==> src/implementation.tex <==
\section{Implementation}\label{sec:implementation}

A prototype of the approach has been implemented.
It is meant to eventually replace the grading system of an existing web plugin.
Due to resource limitations, it has to run client-side.
This suggested to use JavaScript as the programming language, since it is the standard for client-side execution on the web.
The prototype should also have the option to be used as an API or standalone, which meant there would be different build targets.
Additionally, an existing \ac{sql} parser was to be used, instead of implementing a new one, in order to facilitate development.
The npm package "Node \ac{sql} Parser" was chosen for its comprehensiveness and active development / support.
Therefore, npm also serves as the build system for the prototype, with build targets for Node.js and browser.
And in order to have the advantages of a strongly typed language, like type checks at compile time, TypeScript was used and compiled down to JavaScript.


\subsection{Standalone frontend}\label{sec:gui}

For standalone use, a HTML frontend was built, which can be seen in \autoref{fig:frontend}.
It consists of input fields and controls at the top and an output field at the bottom, with a progress bar being the divider in between.

\begin{figure}
	\centering
	\includegraphics[width=\linewidth]{fig/GUI-annotated-2}
	\caption{HTML frontend for standalone use of the prototype.}
	\Description{The frontend contains text fields for the database schema, destination and start queries, as well as for adjusting the cost of every edit individually.}
\label{fig:frontend}
\end{figure}

The left half of the input is more commonly used and partly required.
The first input field is for the database schema.
This is specified in the form of one table per line, consisting of the table name followed by its columns' names enclosed in parentheses, for example \texttt{students(id, name, age)}.
The second input field is for the reference solution, given in \ac{sql}.
It will be the destination query for the shortest path search (see \autoref{sec:search-direction}).
The third one is for the test subject / student-devised solution, also given in \ac{sql}.
It will be the start, from which the destination is to be reached.
Below that are the execution controls, which start or cancel the search process.

The right half is optional configuration.
With the edit configuration, the cost of each edit can be set individually.
There are atomic edits, horizontal edits, and shortcut edits.
The latter two combined make up the shortcut edits as defined in \autoref{sec:edit-set-construction}, but have been separated for easier navigation, due to their large number.
The defining characteristic of horizontal edits is that the nodes / \acp{ast} connected by them always have the same distance from the empty \ac{ast}.
For example, when swapping the positions of two SELECT-elements, the cost of building the respective \ac{ast} from scratch remains unchanged.

Below the edit configuration, a maximum search distance can be specified.
If it is exceeded before reaching the destination, the search is aborted.
This is useful for grading assignments, because there is a maximum number of points.
When the distance exceeds it, no points would be awarded anyway.

The progress bar approximates the progress of the search.
This can only be estimated, because the distance to the destination is not known in advance.
If a maximum search distance is specified, the bar progresses linearly by $\frac{currentDistance}{maxDistance}$.
Otherwise, the bar converges to 100\% based on $1 - exp(-currentDistance)$. %, because the distance could become arbitrarily high.

The feedback output shows the results (see \autoref{sec:result}).
The first line specifies the total distance.
Below that, the shortest path is listed with all of its intermediate steps and the edits between them, ordered from start to destination.


\subsection{Nodes}\label{sec:node-implementation}

Nodes / \acp{ast} generally do not change once created, but their number grows exponentially and most will share (sub)components with others.
Therefore, an immutable data structure design was chosen, since its very idea is to have immutable (sub)components, which are shared between objects to reduce memory costs.
Also, every (sub)component, and therefore the whole \ac{ast}, is hashable.
If two hash values differ, the respective components are guaranteed to not be equal.
This is used as an early rejection condition during comparisons, making them faster.
Additionally, the visited nodes (see \autoref{sec:custom-algorithm}) are stored in a HashMap.
So in order to find out if a node / \ac{ast} has already been visited, it only has to be compared to those with the same hash value, greatly reducing the number of comparisons.

In slight deviation from \autoref{sec:node-definition-and-comparison}, a small form of normalization / canonicalization is used during comparison to reduce the number of different nodes:
An alias assigned to a FROM-clause element only affects how the element is referenced within the query.
But, as long as it is un-ambiguous, it does not change the result of the query, so it does not affect semantic equivalence.
It is also considered irrelevant for grading, what exactly was chosen as the alias.
Only whether there is one or not might be relevant.
This is why the queries in \autoref{lst:query-with-alias} and \autoref{lst:query-with-different-alias} are the same \ac{ast} according to the comparison implementation.
Meanwhile, the query in \autoref{lst:query-without-alias} is semantically equivalent to both, but not considered the same \ac{ast}.

\begin{lstlisting}[language=SQL, caption=\acs{sql} query with alias for the table \texttt{students}., label=lst:query-with-alias]
    SELECT s.id
    FROM students s
\end{lstlisting}

\begin{lstlisting}[language=SQL, caption=\acs{sql} query with different alias for the table \texttt{students}., label=lst:query-with-different-alias]
    SELECT stud.id
    FROM students stud
\end{lstlisting}

\begin{lstlisting}[language=SQL, caption=\acs{sql} query without alias for the table \texttt{students}., label=lst:query-without-alias]
    SELECT id
    FROM students
\end{lstlisting}

\begin{figure}
	\centering
	\includegraphics[width=\linewidth]{fig/AST}
	\caption{\acs{uml} diagram of the currently implemented \acs{ast}.}
	\Description{The implementation mainly follows the syntactic structure of a query, with a maximum of 2 levels of inheritance.}
\label{fig:ast}
\end{figure}

A \ac{uml} diagram of the currently implemented \ac{ast} can be seen in \autoref{fig:ast}.
Some data types and features of TypeScript have been transformed into their \ac{uml}-equivalent.
For example read-only attributes are represented as private attributes with public get-methods.
These, and the fact that all set-methods return a modified copy of the object instead of modifying it directly, are part of the immutable design.
The \texttt{recursivelyReplace}-methods are also a result of this and will be explained in the next section.

The classes are designed to intuitively represent the components of an \ac{sql} query as described in \autoref{sec:sql}:
The root of every \ac{ast} is a \texttt{Query}.
Its WHERE-clause, HAVING-clause and GROUP-BY-elements are simply \texttt{Expression}s.
A \texttt{SelectElement} is implemented as its own class, because it is an expression combined with an optional alias.
Similarly, a \texttt{FromElement} is a table name with an optional alias, as well as a \texttt{JOIN} type (e.g. \texttt{INNER}, \texttt{LEFT}, \texttt{RIGHT}, implemented as an enum) and \texttt{JOIN}-condition expression.
And an \texttt{OrderBy}-element consists of an expression and order-direction, either ascending or descending.

An \texttt{Asterisk}-expression can refer to a specific table name or FROM-element alias.
The same applies to a \texttt{ColumnReference}-expression, which additionally carries the name of the column it is referencing.
\texttt{Not}, \texttt{AggregationFunction}, and \texttt{BinaryExpression} are recursive / nestable because they can contain other expressions.
The \texttt{AggregationFunction} knows its type (e.g. MIN, MAX, AVG) and whether it is DISTINCT (i.e. COUNT(DISTINCT ...)).
The \texttt{BinaryExpression} only knows its type (e.g. \texttt{=}, \texttt{<}, \texttt{>}).

The diagram shows how every component inherits from \texttt{Hashable}.
Its \texttt{hashMax}-value is for parent components with an arbitrary number of children.
For example, when calculating the \texttt{hash}-value of a \texttt{Query}, for every \texttt{SelectElement se} the query's \texttt{hash} is increased: \texttt{hash = hash * se.hashMax() + se.hash()}.
If the children's hashes were simply summed up, without multiplying by their \texttt{hashMax} in between, they would interfere with each other, resulting in many different \acp{ast} with same \texttt{hash}-values.
This way, they are effectively separated.

The \texttt{DepthInfo} is used for ensuring termination and for optimization.
As explained in \autoref{sec:termination-of-algorithm}, the \ac{ast} size needs to be limited to ensure termination.
In terms of optimization, the limit should be as small as possible.
This can be pushed further by choosing individual limits for different types of components, e.g. column-references, aggregation functions, binary expressions, etc..
This way, if certain components are used sparsely or not at all in the destination \ac{ast}, creating them via edits can be constrained as well, greatly reducing the number of generated nodes.
The limits can also be divided the same way by location, for example per query clause.
These optimizations are implemented via \texttt{DepthInfo}, the \texttt{remainingDepth}-method and according checks in the edits.

While the \ac{ast} is already quite extensive, some features are missing.
Most notably, the WITH-clause, the IS NULL operator and NULL, boolean, integer and string constants.
But with the theoretical foundations in \autoref{sec:concept}, implementing these should only be matter of time.


\subsection{Edits}\label{sec:edit-implementation}

There are 156 edits currently implemented, 82 of which are atomic edits.
Each one has a compact unique name for easy identification and a full description in natural language for more intuitive feedback.
While float values as costs are theoretically possible, only integer values can be used in the prototype because this allows to implement the priority queue using discrete buckets.

As mentioned in \autoref{sec:edits-vs-edges}, an edit generally not only needs the query to perform on, but also the database schema and a meta-info.
The schema is required because semantic equivalence, and therefore whether an equivalence edit is applicable, may depend on it (see \autoref{sec:definitions}).
The meta-info is required for ensuring termination, because it contains the maximum \ac{ast} size (see \autoref{sec:termination-of-algorithm}).
This is further used for optimization, like described in the previous section.
The number of generated nodes is reduced by having individual limits per component, as well as per query clause.

The \texttt{recursivelyReplace}-methods are a means of combining these depth limits with the immutable, recursively nestable expressions.
One operation, e.g. inserting an aggregation function, is to be performed at any depth within the expression tree, up until a certain limit.
Also there is not only one, but multiple different aggregation functions that could be inserted, so this operation is not a 1-to-1, but a 1-to-n function, called multimap.
Finally, the operation not only needs the current (sub)expression on which it operates, but also the stack of parent expressions up until this point.
This is because for example aggregation functions cannot be nested within each other.
So one can only be inserted at a certain position within the expression tree, if there is not already one above it.
Hence the format \texttt{recursivelyReplace( multimap, maxDepth )}, with \texttt{multimap} being the operation of the form \texttt{(Expression, stack) => Expression[]}, \texttt{stack} being an \texttt{Expression[]}, and an \texttt{int}-value \texttt{maxDepth}.

A slightly simplified example containing all of the above can be found in \autoref{lst:example-edit}.
The edit object, which is being added to the set of atomic edits, consists of a unique name, full description, integer cost and perform-function.
The latter takes the query to edit, the (here unused) database schema, and a meta-info, as well as a return-parameter.
In it, the operation \texttt{addAggregationFunction} is performed anywhere within the expression tree, up until the maximum depth of \texttt{meta.having.aggregationDepth}.
The \texttt{recursivelyReplaceHaving}-method returns the new HAVING-clauses generated by this.
Finally, these are used to replace the current HAVING-clause, resulting in new ASTs.
These are the neighbors generated by this edit.

\begin{lstlisting}[style=JavaScript, caption=The \texttt{addHavingAggregationFunction} atomic edit implementation., label=lst:example-edit]
addEdit(atomicEdits, {
	name: "addHavingAggregationFunction",
	description: "Add (missing) aggregation function to having-clause",
	cost: 1,
	perform: (query: Query, _schema: Schema, meta: MetaInfo,
			result: Query[]) => {
		if(meta.having.aggregationDepth > 0) {
			const expressions = query.recursivelyReplaceHaving(
				addAggregationFunction, meta.having.aggregationDepth);
			for(let e=0; e<expressions.length; ++e)
				result.push(query.setHaving(expressions[e]));
		}
	}
});
\end{lstlisting}


\subsection{Algorithm}\label{sec:algorithm-implementation}

The shortest path algorithm implementation behaves exactly as described in \autoref{sec:custom-algorithm}.
Its arguments are a destination, a start, a database schema, a (potentially configured) set of edits, and a maximum search distance.
However, only the first one of them is required.
If no start query is provided, the empty \ac{ast} is used as the start.
If no schema is specified and the destination query is completely un-ambiguous, a schema can be deduced from it.
Of course, information not present in the query, e.g. unmentioned columns, will be missing, which might influence the result.
A configured set of edits is not required, because there is a default configuration, which can be used instead.
And if the maximum search distance is not limited, it is infinite.

During initialization, the destination query is checked to be executable in the context of the database schema.
As established in \autoref{sec:search-direction}, while no assumptions or demands can be made for the start, the destination can sensibly be required to be executable.
This is another way of narrowing down the search space, because no incorrect values, references and constructs have to be generated, as long as they are not needed for an intermediate step of a potential shortest path.
This is why, in the previous section, no \acp{ast} needed to be generated where aggregation functions are nested within each other.

This is pushed further by also restricting the database schema depending on which parts of it are actually used in the destination.
Like for the \ac{ast} size, this can also be divided by location.
This limits the possible values, mainly those of table- and column-references, even more.
These restrictions can, however, also not be applied everywhere.
Because for some edits, information about parts of the schema, that are not present in the destination, might be required.
For example, whether adding or removing an element of the ORDER-BY-clause is an equivalence transformation depends on whether it is functionally dependent on a previous element.
And the information about a column being functionally dependent on the primary key of its table would be lost, if said column was removed from the schema for not being present in the destination.
Instead, information about which parts are used in the destination are passed as part of the meta-info.

